CGraph: Graph Based Extensible Predictive Domain Threat Intelligence Platform

Ability to effectively investigate indicators of compromise and associated network resources involved in cyber attacks is paramount not only to identify affected network resources but also to detect related malicious resources. Today, most of the cyber threat intelligence platforms are reactive in that they can identify attack resources only after the attack is carried out. Further, these systems have limited functionality to investigate associated network resources. In this work, we propose an extensible predictive cyber threat intelligence platform called cGraph that addresses the above limitations. cGraph is built as a graph-first system where investigators can explore network resources utilizing a graph based API. Further, cGraph provides real-time predictive capabilities based on state-of-the-art inference algorithms to predict malicious domains from network graphs with a few known malicious and benign seeds. To the best of our knowledge, cGraph is the only threat intelligence platform to do so. cGraph is extensible in that additional network resources can be added to the system transparently.

==> WebConf 2022 Demo cGraph arxiv/abstract.tex <==
 Ability to effectively investigate indicators of compromise and associated network resources involved in cyber attacks is paramount not only to identify affected network resources but also to detect related malicious resources. Today, most of the cyber threat intelligence platforms are reactive in that they can identify attack resources only after the attack is carried out. Further, these systems have limited functionality to investigate associated network resources. In this work, we propose an extensible predictive cyber threat intelligence platform called cGraph that addresses the above limitations. cGraph is built as a graph-first system where investigators can explore network resources utilizing a graph based API. Further, cGraph provides real-time predictive capabilities based on state-of-the-art inference algorithms to predict malicious domains from network graphs with a few known malicious and benign seeds. To the best of our knowledge, cGraph is the only threat intelligence platform to do so. cGraph is extensible in that additional network resources can be added to the system transparently. %Further, cGraph is scalable to support network data spanning a long time period.
 
 %\ravindu{In this paper, we demonstrate the engineering effort of making the cGraph system and possible user scenarios of the cGraph system. And further we show why cGraph system is unique from current available popular systems out there.}
 
 
 

==> WebConf 2022 Demo cGraph arxiv/conclusion.tex <==
We propose, cGraph, which takes domain threat investigation a step forward. cGraph can efficiently store and process large amount of disparate network data, build network graph for any given time period and perform real-time graph inference to predict domains as malicious or benign, compared to reactive threat intelligence platforms available. We demonstrate three frequent use cases of cGraph: domain search, real-time reputation computation and network graph evolution along with the maliciousness scores of domains in the network over time.

%The main purpose of the project was to design and implement a scalable and efficient big data graph system that can process and store a large amount of graph data. The designed system able to process and store the 250 GB - 300 GB of daily data feed within 1-1.5 hours and able to retrieve the necessary information, search queries within seconds. Graph inference system and malicious act discovering system has implemented on top of the designed high available big data processing system. Working accuracy of the inference system has reached 96\% by indicating the system has reached the best prediction capabilities as well as better performance in the overall system.

==> WebConf 2022 Demo cGraph arxiv/demo.tex <==
In this section, we show three common use cases of our system.

\textbf{Searching for impersonating domains and related other malicious domains}:
Attackers increasingly impersonate popular brands such as Apple, Paypal and Microsoft. %Out of all impersonation attacks, combosquatting domains~\cite{Kintis:2017:Combosquatting} are the most prevalent. 
cGraph allows to search for any popular brands and easily identify likely combosquatting domains.%~\cite{Kintis:2017:Combosquatting}.  
  We demonstrate the use case of hunting for combosuqatting domains of paypal.com. 

\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{figures/Screenshot1.png}
\caption{Search results for the keyword paypal}
\label{fig:cp1}
\end{figure}

Figure~\ref{fig:cp1} shows the search results for the keyword paypal ranked based on VT positive counts. An investigator may pick any of these domains to further investigate. Assume that they select paypal-assist.com, which takes them to the graph based interface shown in Figure~\ref{fig:cp2}. This view includes the domain summary information, network graph, Alexa ranking and VT statistics over time, IP geolocation information and historical hosting information.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{figures/Screenshot2.png}
\caption{Dashboard for the domain paypal-assit.com}
\label{fig:cp2}
\end{figure} 

%Figure \ref{fig:cp2}  shows the initial information shown for the domain paypal-assit.com; it includes the domain summary information, network graph, Alexa ranking and VT counts over time, IP geolocation information and Passive DNS information. 

The ability expand the network graph based on the investigator's findings is quite useful in practice. cGraph not only allows to expand any network node when it has children. but also provides real-time predict intelligence on the unknown domains in the network.
%as long as there are additional nodes in the connected component under consideration.
Figure~\ref{fig:cp3} shows the expansion of the IP address 47.254.170.24 that adds 4 additional domains to the graph which are hosted on this IP address. 

\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{figures/Screenshot3.png}
\caption{Expansion of the IP address 47.254.170.24}
\label{fig:cp3}
\vspace{-4mm}
\end{figure} 

The inference graph view shows the maliciousness score of each domain in the network graph %(upto 2 hops from the domain under consideration) based on known seed domains, paypal-assist.com in this case. 
calculated on the fly using the BP algorithm based on known seed domains, paypal-assist.com in this case. Figure~\ref{fig:cp4} shows that cGraph inference identifies the domains google-standard.com, google-money.com, paypal-debit.com and google-sale.com to be highly malicious. %\rev{How exactly? (The screenshots are too small).} \ravindu{should we explain this form image or from an sentence sir}
%Nabeel: BP explained above covers this

\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{figures/Screenshot4.png}
\caption{Malicious domains identified by inference}
\label{fig:cp4}
\end{figure} 

\textbf{Evaluation of maliciousness of any domain via the browser plugin}:
In this use case, we show how cGraph API can be consumed to obtain reputation scores for websites on the fly. While blacklists such as GSB that powers the Chrome browser identify many malicious websites, they are either slow to react or unable to make a judgement if the website content is cloaked from the blacklisting service. cGraph's reputation engine takes a different approach and infers the maliciousness of domains based on the maliciousness of the neighboring network resources such as sibling domains, name servers, CNAME domains, IP addresses and certificates. As mentioned earlier, the reputation score is computed dynamically based on the status of the network infrastructure at the present moment.

\begin{figure}[h]
\centering
\includegraphics[width=0.3\linewidth]{figures/bad.png}
\caption{Browser plugin: real time reputation score}
\label{fig:ce}
\vspace{-4mm}
\end{figure}

Figure \ref{fig:ce} shows the cGraph inference API in action when a user types the website soaponline.org. The maliciousness score indicates how likely the domain is malicious or benign. In this example, the maliciousness score of 0.87 indicates that soaponline.org is highly likely to be malicious. 


\textbf{Investigating the network over time}:
Network resources associated with domains change over time due to both malicious as well as benign reasons. For example, cloud IP rotations, CDN hostings and IP load balancing change IPs associated with domains frequently. Attackers also move from one IP to another as a technique to either resist take down or evade detection. cGraph timeline feature allows to investigate the network graph over a time period. Coupled with the real-time inference feature, one can observe how the reputation of any of the domains change over time. Figure~\ref{fig:day1day2} shows the network graph on day 1 and the evolved network graph on day 7 respectively. This allows the investigator to learn the fluxing behavior %(chaining IP or domain frequently for malicious purposes) 
of domains and take necessary actions.

% \begin{comment}
% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.2\textwidth} 
%     \includegraphics[width=\textwidth]{figures/day1.png}
%     \caption{Timeline: day 1 of example domain, freefacebookhacking.com}
%     \label{fig:day1}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.2\textwidth}
%     \includegraphics[width=\textwidth]{figures/day2.png}
%     \caption{Timeline: day 7 of example domain, freefacebookhacking.com}
%      \label{fig:day2}
%   \end{minipage}
% \end{figure}
% \end{comment}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\linewidth]{figures/day1day2.png}
\caption{Network timeline for day 1 (left) and day 7 (right)}
\label{fig:day1day2}
\vspace{-4mm}
\end{figure}


==> WebConf 2022 Demo cGraph arxiv/introduction.tex <==
Internet domains are the launch pad for many cyber attacks we observe nowadays. One effective way to reduce the damage caused by such attacks is to identify the domains involved early and take actions such as blocking, taking down or sinkholing. Further, these malicious domains have underlying associations with other Internet resources that help to uncover malicious infrastructures. We observe that existing threat intelligence systems 
%\nabeel{Can you add two reference platforms here}\ravindu{Added sir} Ex- 
,such as Cisco Umbrella Investigate\eat{\cite{cisco}} and Anomali\eat{\cite{anomali}}, fail to take advantage of such associations to detect stealthy malicious domains nor do they capture such associations in a user-friendly graphical form that allows users to easily explore related Internet resources. All these solutions are reactive in nature and by the time security operation teams observe them the damage is already done. A predictive solution would immensely assist in mitigating such therats.  Motivated by these gaps in the industry, we  build a proactive threat intelligence platform that can uncover malicious domains early and visualize associated Internet resources in a graph format for easy analysis.
%Nabeel: commented out the references above to save some space

Building an investigation platform in this domain involves a unique set of challenges. First, the amount of data one needs to process on a daily basis is huge. On average, we observe around 850 million network records per day. Second, the network data is highly dynamic. For example, domains change their hosting IPs periodically, the ownership of IPs change over time, new domains are created and existing domains cease to exist. Third, intelligence sources such as Phishtank, VirusTotal and GSB, contain limited information about the status of domain and they are slow to detect malicious domains~\cite{graphinf:2020}. %\ravindu{Shall We cite  USNEIX work sir}. 
%Nabeel: We will cite the graph inference paper instead as it is more appropirate here.
This is due to the fact that most of such systems rely on either website content or user accessing of these websites to ascertain whether they are malicious or not. Providing timely and up-to-date intelligence is thus a challenge on its own. Fourth, network data, though mostly structured, is available in different data formats and these formats over time. Fifth, collecting additional network data and intelligence seeds is often rate limited and encounter frequent network failures. Sixth,  storage and retrieval of huge amounts of graph data, especially in community databases, are not demonstrated to work reliably in practice.

In this work, we build a system called cGraph to address the above mentioned limitations. We design to implement a scalable big data processing pipeline that can ingest billions of disparate reports daily. In order to track the changes over time, we build succinct snapshots of the whole Internet on a daily basis. 
%\ravindu{Should we mention we take the snapshot of DNS formation not traffic or routing, sir }. 
%Nabeel: What you currently have is good.
cGraph provides predictive intelligence by incorporating state of the art graph inference based malicious domain prediction techniques~\cite{graphinf:2020}. In order to make the system oblivious to data format changes, cGraph provides one level of indirection to ingest data as common schema into the system. This allows one to incorporate data format changes without requiring to change the data processing pipeline allowing to extend with additional data sources transparently. Further, unlike prior work~\cite{graphinf:2020} which utilizes static graphs to infer malicious domains, cGraph is able to construct a graph around the domain in question on the fly and generate real-time intelligence. This gives cGraph to predict the maliciousness of any domain provided there are seed domains in the neighborhood. %\ravindu{Which adding the extensibility to the cGraph as an extensible threat intelligent platform. } 
%cGraph is developed using open source software and uses commodity hardware. cGraph uses custom database designs and scalable architecture to store and efficiently retrieve huge amounts of graph data.

\textbf{Demonstration Scenarios}: cGraph assists in domain threat investigation as well as identification of associated malicious domains~\footnote{Demonstrations of a combosquatting domain and a benign domain investigation are available at https://youtu.be/yu47CZkp\_eY and https://youtu.be/waxczBk7vA8 respectively.}. We show three use cases: (1) searching for impersonating domains and discovering related malicious domains, (2) real-time reputation score for a domain via a browser based plugin, and (3) investigation of the evaluation of network resources over time around a domain under consideration. 

%Nabeel: We don't need an outline of the paper as we don't have space.
% \ravindu{I will edit this sir}
% The rest of the paper is organized as follows. Section~\ref{sec:kg} describes the real-world data sources we use and how we construct a knowledge graph incorporating all available network resources. In Section~\ref{sec:archi}, we describe the system architecture from three point of views: infrastructure, data and data flow. Following the architecture, we provide an intuitive explanation of the belief propagation algorithm adapted in our system and its evaluation in Section~\ref{sec:evalinf} and Section~\ref{sec:evalsys} respectively \ravindu{I think we do not have space to explain belief propagation in dedicated chapter}. In Section~\ref{sec:demo} demonstrate three use cases of our system. We critically evaluate and compare our system against prior work in Section~\ref{sec:related}. Finally, in Section~\ref{sec:con}, we conclude our paper.

==> WebConf 2022 Demo cGraph arxiv/network.tex <==
\subsection{Data Sources}
The system ingests four types of data/intelligence sources to build the graph: (1) Farsight Security PDNS~\cite{farsight} - Passive DNS data observed from all around the world which covers the majority of the DNS resolutions in the Internet., (2) VirusTotal (VT)~\cite{virustotal}  - Reputation service that provides aggregated intelligence on any URL, which is the most popular aggregated threat intelligence platform that provides threat reports using more than 80 antivirus engines, blacklists, and sandbox systems., (3) Maxmind \cite{maxmind} - A comprehensive database consisting of geolocations and ASN information of IP addresses (4) Alexa top 1 million domains~\cite{alexa} - Alexa is a widely used resource for search engine optimization and capturing the status of domains. 

In summary, we use Farsight passive DNS records to generate comprehensive knowledge graphs and use Alexa Top 1 million domains, VirusTotal, and Maxmind information to inject the graph with benign and malicious seed domains for running belief propagation and predicting new malicious domains~\cite{graphinf:2020}.

%Table \ref{tab:daily_data} shows the volume and form of the daily feeds and their transformed form after going through the data processing pipelines.
% \begin{table}
% \caption{Structure and volume of daily raw data feeds and transformed data}
% \label{tab:daily_data}
% \begin{tabular}{| p{0.55in} | p{0.55in} | p{0.55in} | p{0.78in}|}
% \hline
% \textbf{Data feed} &
% \multicolumn{1}{l|}{\textbf{Structure of raw data}} &
% \multicolumn{1}{l|}{\textbf{Volume}} &
% \textbf{\begin{tabular}[c]{@{}l@{}}Structure of the \\ transformed data\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Farsight \\ (PDNS)\end{tabular} &
%   Document &
%   170 GB - 195 GB &
%   \begin{tabular}[c]{@{}l@{}}Graph and\\ Time series\end{tabular} \\ \hline
% VirusTotal & Document  & 2.3 GB - 3 GB & \begin{tabular}[c]{@{}l@{}}Document and \\ Time series\end{tabular} \\ \hline
% Alexa Rank & Document  & 18MB          & \begin{tabular}[c]{@{}l@{}}Document and \\ Time series\end{tabular} \\ \hline
% MaxMind    & Key-value & 1 GB - 2 GB   & \begin{tabular}[c]{@{}l@{}}Key-value and\\ Time series\end{tabular} \\ \hline
% \end{tabular}
% \end{table}


% \subsubsection*{Farsight Passive DNS feed}
% PDNS data from Farsight Security is used as the key ingredient of the graph which consists of several types of DNS records such as A, NS, MX, CNAME, and SOA, collected daily. Table \ref{'tab:freq'} shows the volumes of each records type that processed by the system daily. This data source provides this data as a huge flat file in mtbl format. It is extremely time consuming to extract data from these flat files and very difficult to perform lookup queries. Hence, in their raw form, it is difficult to utilize them directly. We prepossess and transform this data into a graph database in order to perform efficient graph retrieval as well as search.
% \ravindu{This tables take more spaces sir, do we keep them or embed the numbers into chapters}
% \begin{table}
% \centering
% \caption{Statistics of PDNS data}
% \label{'tab:freq'}
% \begin{tabular}{| p{0.55in}| p{0.95in}| p{0.85in}|}
% \hline
% Record Type & \begin{tabular}[c]{@{}c@{}}Data Volume (daily)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Number of Records\\(Unique)\end{tabular} \\ \hline
% A           & 68GB-75GB                                                   & 350 million - 400 million                                            \\ \hline
% NS          & 51GB-60GB                                                   & 200 million - 250 million                                            \\ \hline
% MX          & 2GB-3GB                                                     & 10 million - 15 million                                              \\ \hline
% SOA         & 27GB-30GB                                                   & 100 million - 115 million                                            \\ \hline
% CNAME       & \multicolumn{1}{l|}{22GB-25GB}                              & \multicolumn{1}{l|}{100 million - 115 million}                       \\ \hline
% \end{tabular}
% \end{table}

% \subsubsection*{Alexa feed}
% Alexa Rank includes the Alexa rank of Apex/ FQDNs (Fully Qualified Domain Names) based on the popularity and other relevant measurements. This data is used to rank search results as well as to generate benign ground truth for the graph inference algorithm. While popularity does not directly imply that the domain is benign, we identify those domains that stays in the Alexa top ranking for longer period as benign domains. The rationale is that long lived domains with consistently high Alexa ranking requires considerable network resources and investment which attackers are usually declined to do \ravindu{Will add a cite a research paper}.

% %give some insight into initial search results and rank them as well as to be fed to the inference algorithm of the knowledge graph.



% \subsubsection*{VirusTotal feed}
% VirusTotal is a URL reputation system which inspects items with over 70 antivirus scanners and URL/domain blacklisting services and gives a comprehensive report of that URL. cGraph uses VT data as an intelligence source for the inference algorithms in order to predict vertices as malicious or benign. While the schema of VT data gives detailed information about the scanned URL, the system is mainly concerned with the majority vote of the indicators (malicious, spam, phishing, malware, ransomware, suspicious) and the positive count which indicates the number of indicators that have marked the URLs as infected.



% \subsubsection*{Maxmind feed}
% MaxMind is a geo IP locator that gives information of the geolocation of any particular IP. Compared to the other sources, MaxMind brings a considerable amount of data into the system which is easy to manipulate. MaxMind is the main source of geolocation data which gives an insight to the system’s initial search results.



\subsection{Graph Modeling}
To create the knowledge graph (KG), we employ the DNS record types A, NS, MX, SOA, and CNAME, which include the most important information on domains. Specifically, Type A records contain domain to IPv4 address resolutions, Type NS records contain domain to nameserver resolutions, Type MX records contain domain to mail server resolutions, and CNAME records provide domain to alias domains resolutions. All records are created by having a domain name as their pivot. We create a heterogeneous KG utilizing the above DNS records with different edge types representing different record types and nodes representing domains or IP addresses. Our intuition of building such a KG is that attackers are likely to host their domains in the same infrastructure where some of their blacklisted domains are hosted. This allows one to utilize label propagation algorithms to predict malicious domains from a small seed. %building an edge for each DNS record type by using the domain name as the root of the graph smallest connected component. %As shown in the figure [x]

%This structure propagates its connectivity by employing shared resources such as IP addresses, Nameservers, Mailservers, and CNAMEs to link.

%In short, the fundamental goal of constructing the graph is to identify malicious resources and the other beings and malicious resources that are linked to them. Moreover, run the belief propagation as well to find harmful resources ahead of time.

We build a heterogeneous KG based on the following different types of DNS records available in PDNS. %From the different types of records available in the PDNS data (A, NS, MX, CNAME, SOA) the following vertices and edges are extracted into the knowledge graph we build.


\begin{itemize}
    \item Vertices: Apex, FQDNs, IPs, Name Servers, Mail Servers, CNAME, SOA
    \item Edges: Apex-IP, Apex-FQDNs, FQDNs-IP, Apex-NS, FQDNs-NS, Apex-MX, FQDNs-MX, Apex-CNAME, FQDNs-CNAME, Apex-SOA, FQDNs-SOA
\end{itemize}

%Most of the Apex/FQDNs have used the same IPs, name servers, mail servers, and SOA. This gives rise to a large number of connected components with various underlying properties such as the same cloud vendor, CDN, and so on.

%Figure~\ref{fig:hg} shows a simplified instance of a HKG where apex is at the center. 
It is important to store the graph optimized for lookup as cGraph should be able to retrieve the KG for inference as well as replaying of network infrastructure over time quickly. Thus, the graph information is stored along with timestamps at the granularity of a day. %This allows one to efficiently retrieve a graph for a given time period.

% As shown in Figure \ref{fig:hg}, 
%The graph is stored along with time stamp edges which allow one to filter a sub graph as a given any node as center for any given time interval. 

\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{figures/graph (1).png}
\caption{An instance of a HKG}
\label{fig:hg}
\end{figure}
\end{comment}

%To keep the time series changes of the passive DNS graph, designed system builds the graph and stores at the granularity of a day. 

==> WebConf 2022 Demo cGraph arxiv/solutions.tex <==


%\ravindu{Open threat intelligence, TAXII and STIX, and other intelligence systems are introduced decades ago, here we compare the pros and cons of leading threat intelligence platforms out there and why cGraph is a special and novel solution to the game. }

% \begin{table}[!htb]
% \begin{tabular}{|l|l|l|l|}
% \hline
% Platform                             & Description                                                                                                                                                                                                                                                                                     & Pros                                                                                                                                                                                                                                                      & Cons                                                                                                                                                                                                                                                                                               \\ \hline
% AT\&T Cybersecurity                  & \begin{tabular}[c]{@{}l@{}}AT\&T Cybersecurity \textbackslash{}cite\{att\} provides commercial and open source services to manage cyber attacks,\\ including the Open Threat Exchange, \\ which is said to be the world's largest crowd-sourced computer-security platform.\end{tabular}        & \begin{tabular}[c]{@{}l@{}}* Provides detailed threat intelligence on various malware families\\ * Helps protect enterprises from malicious Internet traffic\\ \\ .\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}* No inference on malicious Internet artifacts\\ *  No graph visualization.\end{tabular}                                                                                                                                                                                \\ \hline
% Cisco Umbrella Investigate           & \begin{tabular}[c]{@{}l@{}}Cisco Umbrella Investigate \textbackslash{}cite\{cisco\} gives a complete view of the relationships and evolution of internet domains,\\  IPs, and files which helps to pinpoint attackers’ infrastructures, and expose current and developing threats.\end{tabular} & \begin{tabular}[c]{@{}l@{}}* Provides a detailed historical view of domains based on passive DNS data\\ * Provides information about blocked traffic due to malicious activities.\\ * Provides a maliciousness risk score for each domain.\end{tabular}   & \begin{tabular}[c]{@{}l@{}}* No graph visualization.\\ * Limited information on Internet artifacts such as certificates and IP addresses.\end{tabular}                                                                                                                                             \\ \hline
% VirusTotal Graph                     & \begin{tabular}[c]{@{}l@{}}VirusTotal Graph \textbackslash{}cite\{vt-graph\} is a visualization tool built on top of VirusTotal data set. \\ It explores the relationship between files, URLs, domains, IP addresses and other items encountered in an ongoing investigation.\end{tabular}      & \begin{tabular}[c]{@{}l@{}}* Provides threat intelligence based on 70+ antivirus scanners.\\ * Provides a graph view of the domain under consideration.\\ * Incrementally loads child nodes for parent nodes with many children.\end{tabular}             & \begin{tabular}[c]{@{}l@{}}* Does not provide the capability to dynamically expand or explore graphs.\\ * No inference-based threat intelligence provided.\\ * No intelligence based on certificates or domain registration information.\\ * Unable to traverse graphs based on time.\end{tabular} \\ \hline
% Anomali Threat Intelligence Platform & Anomali \textbackslash{}cite\{anomali\} is a threat intelligence and analysis platform that aggregates threat intelligence data under one platform.                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}* Integrates domain and IP threat intelligence data from multiple sources\\ * Provides a graph representation of Internet artifacts.\\ * Calculates a threat score based on external threat intelligence sources.\end{tabular} & \begin{tabular}[c]{@{}l@{}}* Intelligence is limited to external threat intelligence sources\\ * Unable to dynamically expand and perform a graph-based investigation.\\ * Unable to traverse graphs based on time.\end{tabular}                                                                   \\ \hline
% \end{tabular}
% \end{table}

We thoroughly evaluate the key threat intelligence solutions in the market against cGraph, our threat intelligence platform: AT\&T Cybersecurity, VirusTotal Graph,  Cisco Umbrella Investigate, and Anomali Threat Intelligence Platform. Below, we provide a summary of key differentiation in our system: (1) Dynamic graph-based visualization and search of Internet artifacts for threat intelligence (all the above solutions lack an intuitive graph based navigation), (2) The ability to integrate various data sources and expand the network coverage and the ability to integrate any intelligence sources seamlessly, (3) Predictive domain threat intelligence based on an efficient graph inference algorithm (all above solutions provide only reactive intelligence), and (4) The ability to traverse the network infrastructure based on time and observe the changes in the physical layout as well as the maliciousness of the domains in the network over time, which greatly assist security operation teams in identifying root causes of attacks and the extent of the damage.

==> WebConf 2022 Demo cGraph arxiv/system.tex <==
\subsection{Overall System}
%%Review questions
%\rev{Review questions: How much computing resources does cGraph require?}

%\noindent
%\rev{Review questions: Did you evaluate the performance of your system?}
%\ravindu{Sir, This is tedious to answer, Because system must scale up alone with the volume of the data, And how do we mussers the ratio for that}
%Nabeel: We can exclude this question.

The system consists of four main layers: data processing, database and caching layer, middleware and API layer, and consumer applications. The data processing layer is the component where all the data is cleaned and processed at the first phase. The infrastructure layer orchestrates the resources to insert/update the cleaned and reshaped data into the database cluster. Caching layer handles the data caching and the middleware layer handles the real-time inference process and intermediate data processing tasks.  API layer connects the backend to the consumer products, which are web application, browser extension, and public developer API~\footnote{More information is available at \url{https://qcri.github.io/cgraph/}.}.

%will update the figure
\begin{figure}[h]
\centering
\includegraphics[width=0.6\linewidth]{figures/arch.drawio.png}
\caption{Overall system from infrastructure point of view }
\label{fig:arch}
\end{figure} 


All resources have been provisioned on top of VMware vSphere private cloud. Kubernetes cluster has been installed on top of the provisioned VMs and an abstracted computation resources layer has been created in order to manage all computation resources together.

% The entire application has been built on top of Kubernetes. Web servers, and API (middleware) ingress to the outside world via the load balancers.  Behind that, we have implemented ArangoDB cluster and Greenplum cluster on top of Kubernetes cluster and the Spark cluster has been implemented outside of the Kubernetes cluster. A dedicated set of resources has been allocated to Spark itself to preserve its performance. The middleware has been deployed on top of Kubernetes' via pods as replica sets to preserve the availability and get the maximum use of resources available in the Kubernetes cluster. Apache Airflow was used to automate the daily insertion process by running daily Spark jobs and inserting new data into the database clusters.

% The system functions as a set of microservices. When a search query is executed for an IP, Apex, FQDNs, NS, MX, CNAME or SOA from the frontend of the system, the relevant microservice executes parallel queries on an ArangoDB cluster and fetches the relevant data. If the scanned resource is an IP, the search component interacts with MaxMind IP database and gather necessary data. All other resources will additionally fetch data from the VT profile database and Alexa Rank database. The retrieved results will be sorted based on Alexa Rank and VT feedback. The results will be displayed on the front-end as a ranked list of search results. 

% When a search result is selected, the graph data retrieval endpoint will fetch the data necessary to render the graph in the front-end. Graph data retrieval endpoint consists of two children microservices; a microservice to handle the depth and the number of nodes returned in the graph traversal, and another microservice to handle the traversal of the graph using time property. VT scan and Alexa scan microservices will fetch data relevant to the vertex and assign a maliciousness score to each domain of the graph using the graph inference algorithm.

% The Spark pipeline is designed in a way to work as five parallel Spark jobs, each for processing A, MX, NX, CNAME, and SOA records as indicated in figure \ref{fig:pipe}. Each job is automatically triggered by Airflow with new data for each day. Each pipe has three phases. Phase one cleanses and transforms the raw data into a structured form. Underneath these jobs there are a series of MapReduce operations which is executed to clean the data and do the transformation. In the phase two, the cleaned and transformed data are taken and syncced with data from the daily feed of VirusTotal and it augmenting the labelling process. In the phase three, the data is taken and it undergoes the augmenting process again with Alexa Rank data which adds more value and information to the raw data. Later this data is sent to be stored in the relevant databases. 

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{figures/pipe.png}
% \caption{Spark data pipeline with 3 phases}
% \label{fig:pipe}
% \end{figure} 

\subsection{Graph Inference}
%%Review questions
%\rev{Not knowing much about BP and the difference between homogeneous and heterogeneous graphs, I wonder how you had to adapt the algorithm to handle heterogeneous graphs}

\textbf{Inference}. Belief propagation  (BP) is an iterative algorithm that passes the belief iteratively. In each iteration t, belief propagation algorithm updates the belief value on the node and passes the beliefs (messages) to its neighbors based on the belief values it received from the previous iteration t-1. As mentioned, this interactive process continues until each message value passed by a node to a neighbor node converges to a stable value. The final beliefs are extracted after convergence. % The key idea of belief propagation is that for a given node, if it has more benign nodes associated with it, the likelihood of being benign is high whereas if it has more malicious nodes associated with it, the likelihood of being malicious is high. Likewise, a probabilistic answer to the malicious score of a given node will be computed by belief propagation [figure:\ref{fig:BP}].
%Nabeel: let's exclude the graphs as we need to be careful not mix benign and malicious together in the same vicinity.

\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[width=0.8\linewidth]{figures/inference.png}
\caption{Computing the maliciousness score of a node by inference}
\label{fig:BP}
\end{figure}
\end{comment}

%\noindent
%\rev{How are the experiments conducted?}
% We leverage the belief propagation (BP) algorithm utilized with homogeneous graphs~\cite{manadhata:2014:BP,graphinf:2020} to predict malicious domains in our heterogeneous graphs. We periodically collect those marked by at least two VT scanners as malicious seed and the domains that consistently appear in Alexa top 1 million for the last 1 year as benign seed. After seeding the graph, we execute  BP to label unknown domains in the graph. Our experiments show that our inference based classification achieves a high precision of 92.17\% and high recall of 99.41\%.

\textbf{Execution}. The main idea is to construct a KG on the fly and inject ground truth labels to the KG from credible sources where VT, Alexa, and Maxmind and then run the BP algorithm on top of the knowledge graph by using the labeled values as initial beliefs. It propagates a probabilistic values for each unlabeled domain indicating the maliciousness. For bravity, we explain the execution for a selected example graph. The ground truth extraction process is conducted in two stages; benign ground truth extraction and malicious ground truth extraction. 

For the benign ground truth extraction, Alexa Rank data is used. Alexa Rank data feed for the latest seven consecutive days is taken and the domains with Alexa Rank $\leq10000$ is taken for each day. From this, the unique set of domains %is extracted and the top most 700 Alexa Rank domains are 
is taken as the benign ground truth. Similar to prior research~\cite{compromised}, we observe that  domains with Alexa Rank $\leq10000$ which appear consistently throughout a week are likely to be benign as malicious domains do not live longer than a day or two in Alexa 10K.%is under the assumption that such domains are less likely to be attacker manipulated \cite{compromised}.

For the malicious ground truth, the data from the daily feed of VirusTotal is used. VirusTotal reports for latest seven consecutive days are taken and and the reports with a VT positive count of at least 3 is extracted as malicious ground truth as VT reports with 2 or less positive counts are known to be a less reliable indicator of maliciousness~\cite{graphinf:2020}. We manually verify random samples of benign and malicious ground truth and ascertain that they are indeed correctly labeled. %From this, the unique set of records is taken and a random sample of 600 records was taken as the malicious ground truth.

%After the extraction of malicious and benign seeds, a few random samples were selected in order to carry out manual verification to verify that the extracted samples are correct. It was observed that the sample set had no ambiguous seeds, so the collection of 1300 ground truth data was used to run the inference algorithm and extract the belief value after the inference process was done. 1300 is the size of the ground truth we precisely validated manually for the initial training, and unlike deep learning, statistical machine learning does not converge to higher precision, recall, accuracy rates with more data after the convergence point. 1300 was the roughly measured convergence point of the data set and the precisely validated data within the time.

 After seeding the KG with the ground truth domains, we run a multi-threaded version of the BP algorithm which executes within a few seconds. Our experiments show that our inference based classification achieves a high precision of 92.17\% and high recall of 99.41\%. We observe that a domain's maliciousness score does not affect significantly by considering only its two hop neighbors compared to the complete graph. Hence, for the real-time inference on an unknown domain, we build the two-hop neighborhood KG and run the inference algorithm to further improve the computational performance. 
 %Nabeel: this thinking should work. we will try this on the conference version and report the results. I will provide additional graphs to do so. Also, we should try other inference algorithms such as label propagation and also shallow embeddings as baselines for the conference paper to do a thorough evaluation on graph inference algorithm classification performance and computational performance.
